Towards Supporting Legal Argumentation with NLP: Is More Data Really All You Need?

Modeling legal reasoning and argumentation justifying decisions in cases has always been central to AI & Law, yet contemporary developments in legal NLP have increasingly focused on statistically classifying legal conclusions from text. While conceptually simpler, these approaches often fall short in providing usable justifications connecting to appropriate legal concepts. This paper reviews both traditional symbolic works in AI & Law and recent advances in legal NLP, and distills possibilities of integrating expert-informed knowledge to strike a balance between scalability and explanation in symbolic vs. data-driven approaches. We identify open challenges and discuss the potential of modern NLP models and methods that integrate

==> Text/hybrid.tex <==
%Any data-driven method that leaps straight from natural language description to case outcome classification/prediction without adherence to the reasoning used in the legal domain, will be severely limited in its ability to be adequately audited to meet appropriate standards of explainability and justifiability. This concern is underscored by experimental analyses from prior works that emphasize the risks associated with data-driven approaches focused solely on improving quantitative prediction metrics. For instance, in the study by \citealt{medvedeva2020using}, judges' names alone were used to predict outcomes, yielding notably higher accuracy scores. Similarly, \citealt{santosh2022deconfounding} identified tokens like "mr." and "represented," which, although legally irrelevant, demonstrated statistical predictiveness. These findings underscore the necessity for explanations accompanying predictions, enabling clarity on the reasons behind the model's decisions to ensure accountability in the legal context.

The pressing question is how best to integrate legal knowledge and machine learning so that a system can learn from large volumes of data, whilst retaining crucial domain knowledge that is needed to reason about and explain decisions on legal cases, which gave rise to hybrid approaches. 

Earlier work in this direction is Split Up \cite{stranieri1999hybrid} which is a hybrid system that takes nuanced composition of expert-crafted rules and neural networks trained from data that is faithful to a factor-based model of Australian family law, and which forms an early example of transparent and explainable use of machine learning techniques in legal decision support systems. Later works by IBP+SMILE \cite{ashley2009automatically} also falls under this approach of hybrid system, where the justification or argumentation needs to bridge this conceptual gulf between outcome and facts by the use of legally pertinent legal concepts: issues and factors. 

If we restrict using data-driven techniques to ascribe the input to an approved domain model that captures the relevant legal reasoning, one may strike a balance between performance metrics and grounding and explaining reasoning within the law. This division would also alleviate the knowledge acquisition obstacle in practical deployment of traditional approaches which required for manual analysis of cases into factors for representing the new cases. Thus using data-driven approaches for this intensive task of ascribing factors to cases, while reserving the construction of the domain for experts with the appropriate knowledge, seems the sensible way to allocate resources. 

A step towards such approach is applied to World Intellectual Property Organization (WIPO) domain name dispute cases by \cite{branting2021scalable}. They have trained a model to identify text excerpts in case decisions that correspond to relevant legal concepts in the governing rules: these textual patterns essentially correspond to factors. Given a small sample of decisions annotated with legally relevant factors, their model could predict outcomes of textually described cases and identify the factors that could help to explain the predictions, for example, by indicating the elements of the legal rule that have been satisfied or are still missing.

Similarly, the idea of combining these neural NLP models with structural models of legal inference and argumentation can be witnessed in \cite{holzenberger2021factoring} which apply deep neural model for identifying argument slots from the text of legal rules and find suitable filling elements from fact descriptions. Then they are used along with instantiated schemas which  derive the answer to a question about a case that is coupled with the elements of the legal provision. Similarly, \cite{holzenberger2023connecting} automates the process of translating case into a Knowledge base by leveraging it as information extraction task using neural models and this extraction could leverage the high-quality expert system built on statutes. Thus restricting the use of these blackbox NN models to knowledge acquisition functions such as identifying concept-mentions in the statute and unifying them with entity-mentions in the case text, facilitates interpretability and auditability in the model’s output and aligns with the traditional paradigm of modeling legal reasoning as argumentative inference in synergy with statistical learning. 

In this line of restricting use of neural network models to cognition like functions than for the final outcome, \cite{mumford2022reasoning,mumford2023combining} uses neural models to the task of ascription of factors and issues from legal facts and combines the extracted information with a symbolic domain model, ANGELIC ADFs, which capture the legal knowledge in a domain structured way, to derive the outcome of a case, enabling justifications while maintaining improved performance. 

Contrast to above methods, \citealt{santosh2022deconfounding} devised an expert-informed procedure to enhance the alignment of data-driven models with experts. This involved experts identifying distractors among predictive tokens, and then, through adversarial training, removing the distracting signal from the encodings. Despite efforts to improve alignment with experts, the evaluation was conducted using paragraph importance scores generated by integrated gradients. However, these explanations fell short of providing the ideal justifications one would anticipate from such systems in terms of legal concepts. This suggests a need for further refinement in the explanation mechanisms employed by these models to better align with the nuanced and complex nature of legal reasoning.
